Advancing Volumetric Medical Image Segmentation via Global-Local Masked Autoencoder

Masked autoencoder (MAE) is a promising self-supervised pre-training technique that can improve the representation learning of a neural network without human intervention. However, applying MAE directly to volumetric medical images poses two challenges: (i) a lack of global information that is crucial for understanding the clinical context of the holistic data, (ii) no guarantee of stabilizing the representations learned from randomly masked inputs. To address these limitations, we propose the \textbf{G}lobal-\textbf{L}ocal \textbf{M}asked \textbf{A}uto\textbf{E}ncoder (GL-MAE), a simple yet effective self-supervised pre-training strategy. In addition to reconstructing masked local views, as in previous methods, GL-MAE incorporates global context learning by reconstructing masked global views. Furthermore, a complete global view is integrated as an anchor to guide the reconstruction and stabilize the learning process through global-to-global consistency learning and global-to-local consistency learning. Finetuning results on multiple datasets demonstrate the superiority of our method over other state-of-the-art self-supervised algorithms, highlighting its effectiveness on versatile volumetric medical image segmentation tasks, even when annotations are scarce. Our codes and models will be released upon acceptance.

==> algorithms/data_augmentation.tex <==
\vspace{-5pt}
\begin{algorithm}[H]
    \footnotesize
    \caption{Pseudocode of data augmentation in PyTorch-like style.}
    \label{alg:dataAug}
    \begin{algorithmic}[0]
        \STATE \textcolor{mygreen}{\# \textbf{Input}: volume, global\_scale\_factor, local\_scale\_factor, local\_crop\_numbers, global\_size, local\_size}
        \STATE \textcolor{mygreen}{\$ \textbf{Output}: crops}
		\STATE \textcolor{mygreen}{\# volumn: loading a sample from the 3D CT datasat used for pretraining, which has been processed by spacing, scaleIntensity etc. }
		\STATE \textcolor{mygreen}{\# global\_scale\_factor, local\_scale\_factor: factors to scale the image.}
		\STATE \textcolor{mygreen}{\# global\_crop\_numbers: numbers of cropped volume, e.g., 2. }
		\STATE \textcolor{mygreen}{\# local\_crop\_numbers: numbers of cropped volume, e.g., 8. }
		\STATE \textcolor{mygreen}{\# global\_size, local\_size: size for global and local sub Volume.}
		\STATE
		\STATE \textcolor{mygreen}{\# Define transforms $\tau_1$ for generating local sub-volumes}
		\STATE local\_transform = Compose([
		\STATE \quad\quad RandScaleCropd(local\_scale\_factor), \STATE \quad\quad Resized(local\_size)])	
        \STATE \textcolor{mygreen}{\# Define transforms $\tau_2$ for generating local sub-volumes}
		\STATE global\_transform = Compose([
		\STATE \quad\quad RandScaleCropd(global\_scale\_factor), \STATE \quad\quad Resized(global\_size)])		
		\STATE crops = [] \textcolor{mygreen}{\# Process of generating the expected sub volumes}
		\STATE for iter in range(global\_crop\_numbers):
		\STATE \quad crops.append(global\_transforms(volume))
		\STATE for iter in range(local\_crop\_numbers):
		\STATE \quad crops.append(local\_transform(volume))
    \end{algorithmic}
\end{algorithm}
% \vspace{-10pt}


==> algorithms/pretrained.tex <==
% \vspace{-5pt}
% \begin{algorithm}[H]
%     \footnotesize
%     \caption{Pseudocode of proposed SSL pretraining in PyTorch-like style.}
%     \label{alg:overall}
%     \begin{algorithmic}[0]
%         \STATE \textcolor{mygreen}{\# \textbf{Input}: loader/encoder/decoder/m\_encoder/proj\_m/proj\_s and hyper-parameters etc.}
%         \STATE \textcolor{mygreen}{\# \textbf{Output}: encoder}
%         \STATE \textcolor{mygreen}{\# loader: 3D CT dataloader for pretraining}
%         \STATE \textcolor{mygreen}{\# encoder/decoder/m\_encoder/proj\_m/proj\_s: model used for pre-training/reconstruct/project}
%     	\STATE \textcolor{mygreen}{\# m: momentum factor. mask\_ratio}
%     	\STATE
%         \STATE \textcolor{mygreen}{\# Initialization, encoder with mask ratio, momentum w/o mask ratio}
%         \STATE m\_encoder.params = encoder.params
% %        \STATE
%         \STATE for epoch in range(n\_epochs):
% %    	\STATE \quad\quad \textcolor{mygreen}{\# load a minibatch x, Mask M and labels, mask from the small class}
%     	\STATE \quad\quad for xs in loader: 
%     	\STATE \quad\quad \quad\quad g\_xs, l\_xs = aug(xs) \textcolor{mygreen}{\# augmented with the defined \textit{data augmentation} transform}
%     	\STATE \quad\quad\quad\quad \textcolor{mygreen}{\# Obtain masked global and local feature from encoder with mask\_ratio}
%     	\STATE \quad\quad \quad\quad g\_features, l\_features = encoder.forward([g\_xs, l\_xs], mask\_ratio) 
%     	\STATE \quad\quad\quad\quad \textcolor{mygreen}{\# Reconstruct global and local volume from decoder}
%     	\STATE \quad\quad\quad\quad g\_volume, l\_volume = decoder.forward([g\_features, l\_features]) 
%     	\STATE \quad\quad\quad\quad s\_g\_feature, s\_l\_feature = proj\_s.forward([g\_features, l\_features]) 
% %    	\STATE \quad\quad\quad\quad 
%     	\STATE \quad\quad \quad\quad m\_g\_features = m\_encoder.forward(g\_xs, mask\_ratio=0) \textcolor{mygreen}{\#Obtain global volume feature}    	\STATE \quad\quad \quad\quad m\_g\_features = proj\_m.forward(m\_g\_features) 
%         \STATE \quad\quad\quad\quad \textcolor{mygreen}{\# Optimized with the following losses}
%         \STATE \quad\quad\quad\quad $\mathcal{L_R}$ with [g\_xs, l\_xs, g\_volume, l\_volume] computed by Equation(2) in \textcolor{blue}{Section 3.1}
%         \STATE \quad\quad\quad\quad $\mathcal{L_C}$ with [m\_g\_features, s\_g\_feature, s\_l\_feature] computed by Equation(8) in \textcolor{blue}{Section 3.2}
% 		\STATE \quad\quad\quad\quad $\mathcal{L} = \mathcal{L_R} + \alpha\mathcal{L_C}$ 
% 		\STATE \quad\quad\quad\quad $\mathcal{L}$.backward()
% 		\STATE \quad\quad\quad\quad update(encoder, decoder, proj\_m, proj\_s)
% 		\STATE \quad\quad\quad\quad m\_encoder = (1-m) * m\_encoder.params + m * encoder.params 
%     \end{algorithmic}
% \end{algorithm}

% \vspace{-15pt}
\begin{algorithm}[!bth]
    \caption{The GL-MAE Algorithm}
    \label{alg:overall}
    \begin{algorithmic}[1]
        \REQUIRE An assembly CT dataset of $N$ data without labels.
        % \STATE \textbf{Input}: A assembly CT dataset without labels.
        \ENSURE Pre-trained encoder for downstream tasks.
        % \STATE \textbf{Output:} Pre-trained encoder for downstream tasks.
        \STATE // Sample a micro-batch \textit{X} from CT data each iteration.
        \FOR{$x \text{ in \textit{X}}$}
            % \STATE // Apply the augmentation Algorithm \textcolor{red}{1} in the supplementary materials over micro-batch of CT to obtain global and local views.
            % \STATE // Obtain local and global volumes.
            \STATE $\mathit{t_1, t_2}\sim \mathcal{T}$ // Sample transform 
            \STATE $V_l \gets \{v_l^{i}:v_l^{i}=t_1(x), i\in [1, q]$\}  
            \STATE $V_g \gets \{v_g^{i}:v_g^{i}=t_2(x), i\in [1, p]$\} 
            \STATE // Obtain local and global masked volumes.
            \STATE $\widetilde{V_l} \gets \{\widetilde{v_g^{i}}:v_l^{i}=t_m(v_l), v_l\in V_l$\} 
            \STATE $\widetilde{V_g} \gets \{\widetilde{v_l^{i}}:v_g^{i}=t_m(v_g), v_g\in V_g$\} 
            % \STATE $\widetilde{V}\gets \widetilde{V_l} \cup \widetilde{V_g}$
            \FOR{$v_g \text{ in } \textit{V}_g$}
                \FOR{$\widetilde{v_l}, \widetilde{v_g}, v_l, v_g \text{ in } \widetilde{V_l} \cup \widetilde{V_g}\cup V_l \cup V_g$}
                    \STATE Obtain embeddings $\widetilde{Z_l}$ and $\widetilde{Z_g}$ by \textbf{Eq.1}
                    \STATE Obtain embeddings $y_l$ and $y_g$ by \textbf{Eq.2}
                    \STATE // Reconstruction by \textbf{Eq}.3 and \textbf{Eq.4}.
                    \STATE $\mathcal{L}_\mathcal{R}^l(y_l, v_l)$, $\mathcal{L}_\mathcal{R}^g(y_g, v_g)$ 
                    \STATE Obtain embeddings $E_f$, $E_g$ and $E_l$ by \textbf{Eq.6}.
                    \STATE // Global-to-global consistency by \textbf{Eq.9}.
                    \STATE $\mathcal{L}_\mathcal{C}^{gg}({E}_f, \widetilde{{E}_l})$
                    \STATE // Global-to-local consistency by \textbf{Eq.10}.
                    \STATE $\mathcal{L}_\mathcal{C}^{gl}({E}_f, \widetilde{{E}_g})$ 
                    % \STATE  // 
                    \STATE Calculate the overall loss $\mathcal{L}$.
                    \STATE Update parameters of s($\cdot$) and momentum encoder m($\cdot$) with \textbf{Eq.5}
                    % = $\mathcal{D}(s(\widetilde{v_g};\theta_s))$
                \ENDFOR
            \ENDFOR
            % \STATE Apply  to obtain reconstructed views $\{y_g, y_l\}$ 
            % \STATE // \textcolor{mygreen}{To obtain global and local reconstructed views.}
            % \STATE $y_g, y_l$ // Eq.\textcolor{red}{\ref{eq:y}}
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

==> figures/batchsize_lossweight.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.49\linewidth]{imgs/loss_weight.pdf}
    \includegraphics[width=0.49\linewidth]{imgs/Batch_size.pdf}
    \caption{Left figure: Dice score of GL-MAE on the BTCV validation dataset when only varying the Loss weight $\alpha$ in Eq.~\ref{eq:rephrase_loss}. Right figure: Dice score of GL-MAE on the BTCV validation dataset when only increasing the batch size during pre-training. All model above were pre-trained with 100 epochs for saving time.}
    \label{fig:batchsize_lossweight}
\end{figure}

==> figures/mae_lowresolution_loss.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\linewidth]{imgs/mae_lowresolution_loss.pdf}
    \caption{Loss value of the MAE3D on the BTCV validation dataset, backboned by ViT-B when using the down-sampling input volumes as the input.}
    \label{fig:mae_lowresolution}
\end{figure}

==> figures/maskratio_mae.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\linewidth]{imgs/maskratio_mae.pdf}
    \caption{Dice score(\%) of MAE3D on the BTCV validation when mask ratio varies. All the model were pretrained with 500 epochs with a batch size of 128.}
    \label{fig:maskratio_mae}
\end{figure}

==> figures/reconstruction.tex <==
\begin{figure*}[htb]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/reconstrucition.pdf}
    \vspace{-15pt}
    \caption{Reconstruction results of GL-MAE pretrained for 400, 1000, and 1600 epochs for the same input volume, respectively (Best viewed by zooming).}
    \label{fig:reconstruction}
\end{figure*}

==> figures/segmentationResults_more.tex <==
\begin{figure*}[bht]
   \centering
    \includegraphics[width=1.0\linewidth]{./imgs/supp_visualization_seg_v4.pdf}
    \caption{Visualization of segmentation results on BTCV validation dataset. The label blended with volumetric data (1st row), GL-MAE's
    prediction results (2nd row), MAE3D results (3rd row) and Swin-UNETR (4th row).}
    \label{fig:SegVisualizatoin_more}
\end{figure*}

==> sections/Supp_experiments.tex <==
\section{Experiments}\label{sec:exp}

\subsection{Implementation details}
\noindent\textbf{Datasets.}\label{sec:dataset}
We provide a detailed overview of the datasets that we utilized in our experiments. Consistent with prior research~\cite{chen2023masked,tang2022self}, as outlined in Table~\ref{tab:dataset}, the \textit{BTCV} and \textit{TCIA Covid} datasets were merged to create a pretraining unlabelled dataset $\mathcal{D}$, comprising 746 CT datasets focused on thoracic organs. Prior to being fed to the model, the data was normalized within the range of [0, 1], following a hue value of [-1000, 1000]. For our downstream tasks, we employed five distinct datasets that covered tasks such as multiple organ segmentation, whole heart segmentation, and COVID-19 lesion segmentation. While all other datasets were CT-based, \textit{BraTS} was an MRI dataset for further evaluating the generalization capability of our method. Following~\cite{tang2022self,chen2023masked}, we partitioned the datasets into training and validation subsets, based on the official split provided. However, given that the relevant organs differed across each downstream task, we employed different normalized value ranges.
\input{tables/datasets.tex} 
\input{tables/train_configs}

\noindent\textbf{Finetuning details for GL-MAE.} Within the main manuscript, we have presented the linear and end-to-end segmentation settings for the \textit{BTCV dataset}, along with a description of the training process. Table~\ref{tab:configs} illustrates the various configurations utilized for each dataset. For the semi-supervised setting of the  \textit{BTCV dataset}, the model was trained for 3000 epochs, utilizing a batch size of 4 and a learning rate of 1e-4. For the \textit{MM-WHS dataset}, which is CT-based, the input volume was randomly cropped to [96, 96, 96], and the model was trained for 600 epochs with an initial learning rate of 1e-3 and a batch size of 2. The MRI-based \textit{BraTS dataset} had its input volume randomly cropped to [224, 224, 224], and the model was trained for 300 epochs with an initial learning rate of 1e-4. Due to the high resolution of the input volume, the batch size was set to 1. For the \textit{Covid-19-20 dataset}, the input volume was randomly cropped to [192, 192, 16], and the model was trained for 500 epochs, utilizing a batch size of 4 and a learning rate of 1e-4. Finally, for the \textit{MSD Task 07 dataset}, the input volume was cropped to [96, 96, 96], and the model was trained for 600 epochs with an initial learning rate of 1e-4, using a batch size of 2.


\subsection{COVID-19 lesion segmentation}
CT scans are a widely used tool for diagnosing COVID-19, but there is a scarcity of annotated data to train machine learning models for accurate segmentation of lesions. As shown in Table~\ref{tab:transferCovid19}, we evaluated the efficacy of a proposed method for segmenting lesions on the COVID-19 CT dataset. Our proposed method exhibits improved performance in lesion segmentation, increasing the score from 47.92\% to 49.88\% compared to the baseline and surpassing the competitive MAE3D. GL-MAE incorporates a feature learning approach that considers both global and local levels, leading to a significant improvement in model performance for lesion tasks. These findings suggest that our pre-trained model can capture valuable knowledge from unlabelled CT datasets to enhance disease diagnosis, demonstrating the promising potential of the proposed method in practical clinical settings.
\input{tables/downstream_covid3d_seg.tex}


\subsection{Scaling up the pretraining dataset}
We assess whether GL-MAE can be scaled up to a larger pretraining dataset. Specifically, we employ the \textit{LUng Nodule Analysis 2016 (LUNA16)}\cite{murphy2009large,jacobs2014automatic,setio2015automatic,van2009automatic} dataset in our experiments, which can be obtained from the official website\footnote{\url{https://luna16.grand-challenge.org/Data/}}. Following the preprocessing steps outlined in~\cite{tang2022self}, we supplement the pretraining dataset with 886 additional CTs from LUNA16 to increase its scale. As presented in Table~\ref{tab:btcv_more_data}, we pretrained our proposed method on both the original pretraining dataset and the augmented dataset with LUNA16. Notably, our proposed method exhibited further improvements with the augmented dataset, even when trained for the same number of pretraining epochs.
\input{tables/btcv_more_data}


\subsection{Analysis of hyper-parameters.}
\noindent\textbf{Mask ratio.}
Table~\ref{tab:maskratio} presents the mask ratio of GL-MAE. We also investigated the optimal mask ratio for MAE models with ViT-B and ViT-T backbones, and the experimental results are shown in Figure~\ref{fig:maskratio_mae}. We observed that the best mask ratio for MAE3D is 0.6, which is consistent with the optimal mask ratio for GL-MAE.


\input{tables/maskratio}
\input{figures/maskratio_mae}

\noindent\textbf{Loss weight.} Based on the meanings of the losses, the four part losses \textbf{Eq.11} in the main paper can be grouped into two main categories, namely reconstruction loss $\mathcal{L}_R$,  and global-guided consistency loss $\mathcal{L}_C$. The values of these two loss types are on the same order of magnitude, as follows:
\begin{equation}\label{eq:rephrase_loss}
    \mathcal{L} = \mathcal{L}_R + \alpha\mathcal{L}_C,
\end{equation}
where $\alpha$ is the hyper-parameters to balance between the reconstruction and global-guided consistency loss. We conducted experiments to investigate the effect of increasing the weight of the consistency loss $\alpha$ from 0.1 to 1 and 10, and found that a weight of 1 provided the best results, as shown in Figure~\ref{fig:batchsize_lossweight}.

\noindent\textbf{Batch size.} We conducted an investigation into the impact of batch size on the performance of GL-MAE. Specifically, we tried batch sizes of 64, 128, and 256. As shown in Figure~\ref{fig:batchsize_lossweight}, increasing the batch size during pre-training had a positive impact on the downstream performance, which is consistent with the findings in~\cite{chen2020big}. This is because a larger batch size can provide a more accurate estimation of the overall data and accurate optimization direction.
\input{figures/batchsize_lossweight}


\subsection{Addition analysis of GL-MAE}


\noindent\textbf{Training process.} Figure~\ref{fig:training_process} illustrates the training process of the proposed method. More specifically, Figure~\ref{fig:training_process}(a) displays the final training loss curve, comprised of the reconstruction loss $L_R$, and the global-guided consistency loss function $L_C$. It is observed that the loss stability decreases as the number of epochs increases until 1000, and the dice score of the GL-MAE achieves 82.01\% on the BTCV validation dataset. When the model was further pretrained to 1600 epochs, the dice score could result in 82.33\%. Additionally, Figure~\ref{fig:training_process} indicates that the learning rate was adapted using a cosine scheduler.
\input{tables/training_process}

\input{figures/reconstruction}
\noindent\textbf{Reconstruction results.} This study presents examples of slices from CT scans that depict masks and their corresponding reconstruction results. These results were generated using our proposed method, which was pre-trained with 400, 1000, and 1600 epochs, as illustrated in Figures~\ref{fig:reconstruction}, respectively. These figures illustrate both global and local views for various input volumes, with each row consisting of two global views on the left column and six local views on the right column. All of the depicted slices pertain to distorted samples with a high mask ratio of 75\%. As illustrated in Figure~\ref{fig:reconstruction}, while the GL-MAE pertains to more epochs, the reconstruction for global and local views recovers the miss information better (Row 3$\sim$Row5). Our proposed method is capable of simultaneously reconstructing both local and global views, which is consistent with the MAE3D. As the model was trained for more epochs, the global and local reconstruction loss decreased and converged, leading to reconstruction results that were closer to the original data.




% \subsection{Visualization}
% 
% More visualization results could be found on Figure~\ref{fig:SegVisualizatoin_more}.
% \input{figures/segmentationResults_more.tex}

==> sections/Supp_limitation_boarder.tex <==
\section{Discussion}

\subsection{Impact of directly down-sampling the input volume as the input for MAE3D.}
We down-sampled the original sub-volumes to a sub-
volume of [96, 96, 96] and used it to pre-train the MAE. As shown in Figure~\ref{fig:mae_lowresolution}, the loss value of the down-sampling method decreased initially, similar to the cropped approach (used in our method and MAE3D baseline in our paper.), but was unable to continue decreasing the loss. This may be due to two factors. Firstly, the input volume was down-sampled too much from origin input volume (512 × 512 × 128 to 96 × 96 × 96), resulting in significant changes across different patches, making it difficult to recover based on neighboring patches. Secondly, too many details were lost, but the
changes inside the patches were still substantial. These factors made the mode hard to recover the missing pixel well. We also evaluated the performance of the down-sampling method on the BTCV validation dataset. We tried learning
rates of 3e-4, 1e-4, 5e-5, and 1e-5, and found that only a very low learning rate could prevent the model from experiencing gradient explosion and training failure. The results are pre-
sented in Table~\ref{tab:downsampleMAE}, which indicate that the down-sampling method performed significantly worse than the cropped approach used in our MAE3D baselines in the main paper and
our GL-MAE.
\input{figures/mae_lowresolution_loss}
\input{tables/downsampleMAE}

  
\subsection{Broad impact}
Due to recent technological advancements in volumetric medical data sensing, there has been a surge of interest in machine learning algorithms that can perform analysis tasks on such data, as well as a growing number of applications for 3D imaging in fields such as Robotics and Medical Imaging~\cite{an2020ct}. This study focuses on the development of novel yet simple 3D deep learning pretraining algorithms for medical imaging in response to the pressing need for instant analysis systems that can aid the medical community in disease prevention, early detection, diagnosis, and treatment. Medical imaging plays a critical role in healthcare, and with the digitization of medical images, the hope that physicians can instantly analyze them with machine learning algorithms is becoming a reality. This is especially important in the current global pandemic, where radiography images provide a quick and rich diagnosis tool. However, the sheer expense of expert annotation required for supervised machine learning algorithms presents a challenge. To address this challenge, Self-Supervised approaches for representation learning from unlabelled data are necessary. The aim of this study is to provide the necessary tools for 3D image analysis and to aid physicians and radiologists in their diagnostic tasks from 3D scans while reducing the effort and cost of annotation required by these practitioners. Ultimately, this work is a small step towards leveraging machine learning for good in healthcare.


\subsection{Limitations and future work}
The foundation model is a widely recognized approach that exemplifies the potential of big data and large models\cite{touvron2023llama}. Self-Supervised Learning also benefits from the increasing volume of data and model capacity\cite{he2019moco}.
The limitation for GL-MAE is that the design of GL-MAE is relatively complex and may not be straightforward to scale to a larger datasets with higher capacity models, e.g., 100,000 CTs with ViT-Large. This is because the online encoder is fed by multiple masked local and global sub-volumes, and the model has four part losses, which need to tuned and results in expensive computation.

In future studies, we intend to extend our proposed method to larger datasets and higher-capacity models. While our research mainly focuses on pretraining method for downstream segmentation tasks, which are of significant interest to the medical community and have practical utility, we plan to conduct further investigations into other medical tasks, such as disease classification and lesion localization. Finally, we aim to broaden the scope of our framework to include cross-modality medical image analysis.

% \input{figures/reconstruction_e400}
% \input{figures/reconstruction_e1000}
% \input{figures/reconstruction_e1600}

==> sections/Supp_methods.tex <==
\section{Method}\label{sec:supp_method}

We are providing additional information on the implementation of our proposed Global-local Masked Autoencoder. The first section provides a detailed explanation of our proposed algorithm, while the second section outlines and discusses the data augmentation process involved in our method.


\subsection{GL-MAE pre-training}
Algorithm~\ref{alg:overall} provides a step-by-step description of the key processes involved in our proposed method. Firstly, we initialized the momentum encoder with the student encoder and updated it in each iteration with a momentum ratio that is determined by a cosine scheduler. Next, let $\{\tau_1, \tau_2, \tau_m\} \subset\mathcal{T}$ represent the processing described in Algorithm~\ref{alg:dataAug}, and then we apply $\mathcal{T}$ to each input volume and generate both global and local views. These views were then fed into the encoder and momentum encoder for feature extraction. After obtaining their features, we utilized the proposed Global and Local Reconstruction loss functions and Global-guided Consistency Learning loss function to regulate the training process of the model. The momentum encoder would be updated based on the encoder with a momentum ratio $\mu$, which the initial value is 0.996 and increases to 1 during training with a cosine schedule.
\input{algorithms/pretrained}


\noindent\textbf{Why don't directly use Global views as the input for MAE3D?}
The reason for not using Global views directly as the input for MAE3D is that volumetric data, such as CT scans, are typically large in size and need to be broken down into several patches for further processing. Additionally, the reconstruction task for MAE3D is to predict the missing value in a pixel, and downsampling the input volume can result in low resolution and the loss of important details, particularly in small organs and tumors. Therefore, previous work has used cropped volumes from the input volumes to maintain resolution and details. We conducted experiments to analyze the impact of downsampling the input volumes and using them as input. Please refer to Table~\ref{tab:downsampleMAE} in Section Discussion for more information.


\subsection{Data augmentation in the pre-training stage}
Algorithm \ref{alg:dataAug} described the detailed implementation of the data augmentation process. We designed two distinct procedures $\tau_1$ and $\tau_2$ for data augmentation that cater to local and global views. To obtain a global view, we apply $\tau_2$ by first establishing a $\rm{global\_scale\_factor}$  within the range of [0.5, 1] and cropping a sub-volume by a random $\rm{global\_scale\_factor}$. Additionally, we set $\rm{global\_size}$ to [160, 160, 160] and \textit{downsample} the input volume to this size. For the local view, we apply $\tau_1$ by setting a $\rm{local\_scale\_factor}$ within the range of  [0.25, 0.5] and then crop a sub-volume by a random $\rm{local\_scale\_factor}$. Finally, we set $\rm{local\_size}$ to [96, 96, 96] and resize the local cropped sub-volume to this size. For each input volume $x$, we apply the data processing operation $p$ times and $q$ times to obtain $p$ global views and $q$ local views, respectively. To obtain the masked sub-volumes $\widetilde{V}$, following ~\cite{chen2023masked}, we apply $\tau_m$ by randomly masking the patches from the local and global sub-volumes. 

\input{algorithms/data_augmentation}


\noindent\textbf{How much overlap between the local and global views?}
To ensure consistency learning between the local and global views, it is important that they share an overlap region. To determine the overlap region ratio between the local and global views generated from the same data during one epoch of training, we conducted an analysis, and the results are presented in Table~\ref{tab:gl_ratio}. We carefully selected hyper-parameters, including randomly selecting a scale ratio to scale the input data, to ensure that the overlap ratio between the local and global views is reasonable. The average overlap ratio (\%) for the local view $\rm{Overlap}$ was computed over all $q$ local crop $v_l$ global crop $v_g$ for the unlabelled dataset $\mathcal{D}$ with $N$ input data during one epoch using the following equation:

\begin{equation}\label{localview_ratio}
    \rm{Overlap}(\mathcal{D}):=\frac{1}{N|V_g||V_l|} \sum_{i=1}^{N} \sum_{v_g^i\in V_g} \sum_{v_l^i\in V_l}\frac{v_l^{i} \cap v_g^{i}}{v_l^{i}} \times 100.
\end{equation}
Table~\ref{tab:gl_ratio} demonstrates that the global view remains stable at $377\times296\times53$, while the shape of the local view varies from $126\times99\times18$ to $252\times197\times36$ as the $\rm{local\_scale\_factor}$ is modified. Additionally, as the $\rm{local\_scale\_factor}$ is increased from 0.25 to 0.5, the overlap ratio for local $\rm{overlap}$ increases from 62.57\% to 70.00\%. It can be concluded that the local and global views will share the overlap region most of the time, thereby ensuring semantic consistency. To enhance the model's ability to learn robust representation, we adopted a strategy of randomly selecting $\rm{local\_scale\_factor}$ each iteration from the range of [0.25, 0.5]. 

For a more intuitive observation of the overlap situation between the local and global views from the same data, we define a measurement method called $\textrm{Hit}$ in the equation:
\begin{equation}\label{eq:hit}
    \rm{Hit}(\mathcal{D}):= \frac{1}{N} \sum_{i=1}^{N} \sum_{v_g^i\in V_g} \sum_{v_l^i\in V_l} \frac{sgn(v_l^{(i)} \cap v_g^{(i)})}{|V_l||V_g|} \times 100
\end{equation}
\jiaxin{where the $sgn$ represents the Sign function. The 
$\rm{Hit}$ metric can be utilized to measure the frequency of overlap across the entire dataset. It can be observed from the 4th row in Table~\ref{tab:gl_ratio} that the overlap between the global and local views from the same volume is most frequent when we increase the  $\rm{local\_scale\_factor}$}.
\input{tables/supp_gl_ratio}





==> sections/Supp_visualization.tex <==
\section{Visualization}\label{sec:visualization}
More visualization results could be found on Figure~\ref{fig:SegVisualizatoin_more}.
\input{figures/segmentationResults_more.tex}

==> tables/btcv_more_data.tex <==
\begin{table}[htb]
    \centering
    \caption{Dice score(\%) on the BTCV validation dataset by our proposed method under end-to-end segmentation evaluation. ViT-B is adopted and used as the backbone. Both models were trained for 400 epochs.}
	\vspace{-8pt}
    \label{tab:btcv_more_data}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
        \whline
        \multicolumn{3}{c}{Pretraining dataset} & \multirow{2}{*}{Dataset scale} & \multirow{2}{*}{Dice score(\%)} \\
        BTCV & TCIA-Covid19 & LUNA16 &  & \\
        \hline
        \checkmark & \checkmark & - & $\sim 1,000$ & 79.70 \\
        \checkmark & \checkmark & \checkmark & $\sim 2,000$ & 81.41\greenp{1.71$\uparrow$}\\
        \whline
    \end{tabular}}
\end{table}

==> tables/datasets.tex <==
\begin{table*}[thb]
	\centering
	\caption{The datasets used for pre-training and downstream fine-tuning include volumetric data of multiple organs.}
	\label{tab:dataset}
    \resizebox{0.88\linewidth}{!}{
	\begin{tabular}{ccccccc}
        \whline
		Datasets & Organ details & Modality & Train & Validation & Normalized Value \\
		\hline
		\textbf{\textit{Pre-training}} & & & & &\\
		BTCV~\cite{landman2015miccai} & Multiple chest organs & CT & 24 & - & [-1000, 1000]\\
		TCIA Covid19~\cite{an2020ct} & Multiple chest organs & CT & 722 & - & [-1000, 1000]\\
		\cdashline{1-6}
		\textbf{\textit{Fine-tuning}}  & & & & &\\
		BTCV~\cite{landman2015miccai} & Multiple chest organs & CT & 24 & 6 & [-175, 250] \\
		MSD Task 07~\cite{simpson2019large} &  Spleen & CT & 41 & 20 & [-57, 164]\\
		MM-WHS~\cite{zhuang2018multivariate} & Whole heart & CT & 16 & 4 & [0, 1700]\\
		BraTS~\cite{simpson2019large} & Brain tumor & MRI & 484 & 266& -\\ 
		Covid-19-20~\cite{roth2022rapid} & Chest diseases & CT& 160 & 39 & [-1000, 500]\\
        \whline
	\end{tabular}
 }
    % \\ \textsuperscript{*}{\raggedleft{Note: Spl: spleen, RKid: right kidney, LKid: left kidney, Gall: gallbladder, Eso: esophagus, Liv: liver, Sto: stomach, Aor: aorta, IVC: inferior vena cava, Veins: portal and splenic veins, Pan: pancreas, AG: left and right adrenal glands.}.}
    % MM-WHS contains 7 classes, including myocardium of LV (Myo), left ventricle (LV), left atrium (LA), right atrium (RA), right ventricle (RV), whole aorta (aorta) and pulmonary artery (PA)}
 
\end{table*}


==> tables/downsampleMAE.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{c|c}
        \whline
        Operation & Dice score(\%)\\
        \hline
         Cropped& \textbf{81.74}\\
         Downsample& 36.68 \\
        \whline
    \end{tabular}
    \caption{Dice score(\%) performance of the cropped and downsampling operation on the input volume. All model were evaluated under the same split and settings, including pre-trainng and fine-tuning epochs.}
    \label{tab:downsampleMAE}
\end{table}

==> tables/downstream_covid3d_seg.tex <==
\begin{table}[htb]
    \centering
   % \vspace{-5pt}
    \caption{Comparison on Covid-19 CT segmentation dataset with ViT-T as the backbone.}
    \label{tab:transferCovid19}
	\vspace{-5pt}
%	\scriptsize	
    \resizebox{0.75\linewidth}{!}{
    \begin{tabular}{cccc}
        \whline
        Method & Baseline & MAE3D & Ours \\
                \hline
        Dice Score(\%) &  47.92 & \underline{49.52} & \textbf{49.88}\\
        \whline
    \end{tabular}}
   \vspace{-5pt}
\end{table}


==> tables/maskratio.tex <==
\begin{table}[htb]
    \centering
    \caption{Dice score(\%) of BTCV dataset varying mask ratio.}
    \vspace{-8pt}
    \resizebox{0.64\linewidth}{!}{
    \begin{tabular}{c|ccc}
        \whline
         Mask ratio &  0.5 & 0.6 & 0.7\\
         \hline
         Dice score (\%) & 81.53 & \textbf{82.33} & 81.27\\ 
        \whline
    \end{tabular}
    }
    \label{tab:maskratio}
    \vspace{-5pt}
\end{table}

==> tables/supp_gl_ratio.tex <==
\begin{table}[h]
    \centering
    \caption{Average patch size, Overlap(\%), and Hit(\%) of the local and global view from the same input data for one epoch when varies the $\rm{local\_scale\_factor}$.}\label{tab:gl_ratio}
    % \small
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{ccccc}
         \whline
         Metric & 0.25 & 0.5 & 0.25$\sim $0.5 \\ 
         \hline
        Global size & $381\times297\times54$ & 
        $377\times296\times53$ &
        $377\times296\times53$\\
        Local size& $126\times99\times18$ & 
        $252\times197\times36$ & $189\times148\times27$\\
         \hline
         % \multirow{1}{*}{Overlap}& Global & $2.46\pm1.65$ & $4.45\pm2.57$ & $11.15\pm5.15$ & $21.63\pm8.11$ & $8.82\pm5.56$\\
         Overlap(\%) & $62.57\pm36.69$ & $70.00\pm24.13$& $66.89\pm30.00$\\
         % \hline
         \cdashline{1-5}
         Hit(\%) & 89.51 & 100 & 97.12\\
         % & Local view & 100 & & & & \\
         \whline\\
    \end{tabular}
    }
\end{table}


% Factor 0.25, 0.5, 0.25~0.5
% x,y,z
% remove overlap global


% \begin{table}[h!]
%     \centering
%     \caption{Average View size, Overlap(\%), and Hit(\%) of the local and global view from the same input data for one epoch when varies the $\rm{local\_scale\_factor}$.}\label{tab:gl_ratio}
%     \small
%     \resizebox{14cm}{!}{
%     \begin{tabular}{ccccccc}
%          \whline
%          Metric & Factor & 0.25 & 0.3 & 0.4 & 0.5 & 0.25$\sim $0.5 \\ 
%          \hline
%         \multirow{2}{*}{Size} & Global & $176.60\pm32.10$ & $177.02\pm30.92$ & $177.38\pm31.86$& $177.38\pm31.86$ & $177.38\pm31.86$\\
%          & Local & $60.10\pm7.92$ & $72.13\pm9.51$ & $95.90\pm12.72$& $119.45\pm15.90$ & $88.57\pm15.74$\\
%          \hline
%          \multirow{2}{*}{Overlap}& Global & $2.46\pm1.65$ & $4.45\pm2.57$ & $11.15\pm5.15$ & $21.63\pm8.11$ & $8.82\pm5.56$\\
%          Overlap & Local & $62.57\pm36.69$ & $65.95\pm33.62$ & $69.76\pm28.20$ & $70.00\pm24.13$& $66.89\pm30.00$\\
%          % \hline
%          \cdashline{1-7}
%          Hit & - & 89.51 & 94.27 & 99.3 & 100 & 97.12\\
%          \whline\\
%     \end{tabular}}
% \end{table}

==> tables/train_configs.tex <==
\begin{table*}[htb]
    \centering
    \caption{The training details for the model on each dataset mostly followed the settings in the previous works.}
    \label{tab:configs}
    \resizebox{0.75\linewidth}{!}{
    \begin{tabular}{c|cccccc}
        \whline
         Config & Stetting & Learning Rate & Batch Size & Epochs & Cropped Size\\
         \midrule
         BTCV & Linear & 3e-4 & 4 & 3000 & $[96, 96, 96]$ \\
         BTCV & End-to-end & 3e-4 & 4 & 3000 & $[96, 96, 96]$ \\
         BTCV & Semi-Supervised & 1e-4 & 4 & 3000 & $[96, 96, 96]$ \\
         MM-WHS & End-to-end & 1e-3 & 2 & 600 & $[96, 96, 96]$ \\
         BraTS & End-to-end & 1e-4 & 1 & 300 & $[224, 224, 144]$\\
         Covid-19-20 & End-to-end & 1e-4 & 4 & 500 & $[192, 192, 16]$ \\
         MSD Task 07 & End-to-end & 1e-4 & 2 & 600 & $[96, 96, 96]$ \\
        \whline
    \end{tabular}}\\
    % \textsuperscript{*}{\raggedleft{MM-WHS contains 7 classes including myocardium of LV (Myo), left ventricle (LV), left atrium (LA), right atrium (RA), right ventricle (RV), whole aorta (aorta) and pulmonary artery (PA)}}
\end{table*}


==> tables/training_process.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/training_process.pdf}
    \vspace{-15pt}
    \caption{End-to-end segmentation performance on BTCV validation dataset when the pre-training epochs increase.}
    \label{fig:training_process}
\end{figure}
